EvIcon: Designing High-Usability Icon with Human-in-the-loop Exploration and IconCLIP

Interface icons are prevalent in various digital applications. Due to limited time and budgets, many designers rely on informal evaluation, which often results in poor usability icons. In this paper, we propose a unique human-in-the-loop framework that allows our target users, i.e., novice and professional UI designers, to improve the usability of interface icons efficiently. We formulate several usability criteria into a perceptual usability function and enable users to iteratively revise an icon set with an interactive design tool, EvIcon. We take a large-scale pre-trained joint image-text embedding (CLIP) and fine-tune it to embed icon visuals with icon tags in the same embedding space (IconCLIP). During the revision process, our design tool provides two types of instant perceptual usability feedback. First, we provide perceptual usability feedback modeled by deep learning models trained on IconCLIP embeddings and crowdsourced perceptual ratings. Second, we use the embedding space of IconCLIP to assist users in improving icons' visual distinguishability among icons within the user-prepared icon set. To provide the perceptual prediction, we compiled IconCEPT10K, the first large-scale dataset of perceptual usability ratings over $10,000$ interface icons, by conducting a crowdsourcing study. We demonstrated that our framework could benefit UI designers' interface icon revision process with a wide range of professional experience. Moreover, the interface icons designed using our framework achieved better semantic distance and familiarity, verified by an additional online user study.

==> cgf_metadata.tex <==
% \title[EvIcon: Designing High-Usability Icon with Human-in-the-loop Exploration and IconCLIP]%
%       {EvIcon: Designing High-Usability Icon with Human-in-the-loop Exploration and IconCLIP}
\ifthenelse{\equal{\doc}{main}}{
\title{EvIcon: Designing High-Usability Icon with Human-in-the-loop Exploration and IconCLIP}
}
{
\title{Supplemental Material for EvIcon: Designing High-Usability Icon with Human-in-the-loop Exploration and IconCLIP}
}
% \author[paperxxxx]{paperxxxx}

\author[I-Chao Shen et al.]
{\parbox{\textwidth}{\centering I-Chao Shen$^{1}$ ~ Fu-Yin Cherng$^{2}$\thanks{Corresponding author} ~ Takeo Igarashi$^{3}$ ~ Wen-Chieh Lin$^{4}$ ~ Bing-Yu Chen$^{5}$
        }
        \\
% For Computer Graphics Forum: Please use the abbreviation of your first name.
{\parbox{\textwidth}{\centering $^1$ ichaoshen@g.ecc.u-tokyo.ac.jp
, The University of Tokyo, Japan \\
$^2$ fuyincherng@cs.ccu.edu.tw, National Chung Cheng University, Taiwan \\
$^3$ takeo@acm.org, The University of Tokyo, Japan \\
$^4$ wclin@cs.nycu.edu.tw, National Yang Ming Chiao Tung University, Taiwan \\
$^5$ robin@ntu.edu.tw, National Taiwan University, Taiwan \\
%        $^2$ Another Department to illustrate the use in papers from authors
%             with different affiliations
      }
}
}

% Fuyin Cherng\IEEEauthorrefmark{1}, Yu-Ting Wang, Takeo Igarashi, Wen-Chieh Lin,\\ and Bing-Yu Chen

==> conf_preamble.tex <==
\RequirePackage{ifthen}
\newcommand{\conf}{cgf}
% submit, camera, final....
\newcommand{\stage}{final}
% main, supp
\newcommand{\doc}{main}
% \newcommand{\doc}{supp}
% \newcommand{\track}{journal}
% \def\conf{cvpr}
% \input{siggraph_preamble}
\newcommand{\isequal}[3]{
    \ifthenelse{\equal{#1}{#2}}{
        #3
    }{}    
}

\isequal{\conf}{siggraph}{\input{siggraph/siggraph_preamble}}
\isequal{\conf}{cvpr}{\input{cvpr/cvpr_preamble}}
\isequal{\conf}{eccv}{\input{eccv/eccv_preamble}}
\isequal{\conf}{uist}{\input{uist/uist_preamble}}
\isequal{\conf}{chi}{\input{chi/chi_preamble}}
\isequal{\conf}{pg}{\input{cgf/cgf_preamble}}
\isequal{\conf}{cgf}{\input{cgf/cgf_preamble}}
% \isequal{\conf}{tvcg}{\input{ieeetrans/ieeetrans_preamble}}

% \ifthenelse{\equal{\conf}{siggraph}}{
%     \input{siggraph/siggraph_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{cvpr}}{
%     \input{cvpr/cvpr_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{eccv}}{
%     \input{eccv/eccv_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{uist}}{
%     \input{uist/uist_preamble}
% }
% {
% }

==> fig_files/demographic_result_fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/elder_result.pdf}
    \caption{
    % \todo{make the text smaller.}
    Revised icons using \name~show better usability (``AMT rating'') for elder crowdworkers than those revised without \name.
    The results aligned with the perceptual usability feedback for elders provided by \name.
    We labeled the higher ratings in \textbf{green} and the lower ratings in \textbf{red}. 
    }
    \label{fig:revision_process_elder}
\end{figure}

==> fig_files/vis_dist_evaluation_fig.tex <==
\begin{figure}[t!]
\centering
  \includegraphics[width=\linewidth]{figures/raster_all_icon_dist.pdf}
  \caption{
  \iccmt{Remove this..}
The embedding space of the icons for our (a) training and (b) testing samples, where each dot represented an icon, and the color of a dot indicates the function of the icon.
Some icons of functions without established design pattern (\eg~``Archive'' in brown) scattered to the region of other functions.
% (highlighted by the red dot rectangles). 
}
\label{fig:umap_embed}
\end{figure}

==> fig_files/vis_distinct_fig.tex <==
\begin{figure}[t!]
\centering
  \includegraphics[width=\linewidth]{figures/visual_training.pdf}
  \caption{
      \textbf{Training procedure for visual distinguishability.}
      In the training process, we include (a) positive (icons represent the same function) and (b) negative (icons represent different functions) paired examples.
      In each iteration, we encourage the positive paired icons to come closer while the negative paired icons to stay apart from each other.
    }
\label{fig:vis_distinct}
\end{figure}


==> latexmkrc <==
# --- This file allows you to quickly change the style in case you need to resubmit
$ENV{'TEXINPUTS'}='./cvpr//:./eccv//:./cgf//:' . $ENV{'TEXINPUTS'}; 
$ENV{'BSTINPUTS'}='./cvpr//:./eccv//:./cgf//:' . $ENV{'BSTINPUTS'};

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> method.tex <==
\section{Method}
